Progressive Augmentation of GANs

Training of Generative Adversarial Networks (GANs) is notoriously fragile, requiring to maintain a careful balance between the generator and the discriminator in order to perform well. To mitigate this issue we introduce a new regularization technique - progressive augmentation of GANs (PA-GAN). The key idea is to gradually increase the task difficulty of the discriminator by progressively augmenting its input or feature space, thus enabling continuous learning of the generator. We show that the proposed progressive augmentation preserves the original GAN objective, does not compromise the discriminator's optimality and encourages a healthy competition between the generator and discriminator, leading to the better-performing generator. We experimentally demonstrate the effectiveness of PA-GAN across different architectures and on multiple benchmarks for the image synthesis task, on average achieving ~3 point improvement of the FID score.

==> method.tex <==
\section{Progressive Augmentation of GANs} \label{sec:PAGAN}
In \cite{goodfellow2014generative} GAN training is linked to minimizing the Jensen-Shannon (JS) divergence between the data $\mathbb{P}_{\mathrm{d}}$ and generative model distributions $\mathbb{P}_{\mathrm{g}}$ defined on a compact metric space $\mathcal{X}$ such as the image space $[-1,1]^N$ of dimension $N$. Alternatively, we propose to augment the sample \mbox{$\bvec{\vx}\in\mathcal{X}$} or its learned representation with a random bit sequence $\bvec{\vs}\in\{0,1\}^l$ in such way that the original GAN training problem can be casted as minimizing the divergence between two joint distributions of $(\bvec{\vx},\bvec{\vs})$ defined on the augmented space. For computing the divergence, we adopt the adversary process introduced by~\cite{goodfellow2014generative}, while the proposed augmentation is inspired by the information theory view of JS divergence. Both of them are firstly reviewed in Sec.~\ref{subsec:background} to lay the theoretical groundwork for our approach. We further introduce a single-level augmentation in Sec.~\ref{subsec:1-level_aug} and extend it to progressive multi-level augmentation in Sec.~\ref{subsec:multi-level_aug}. 


\subsection{Theoretical Background}\label{subsec:background}


In the context of GANs, $\mathbb{P}_{\mathrm{g}}$ is commonly induced by a function $G$ that maps a random noise vector $\bvec{\vz}\sim\mathbb{P}_{\mathrm{z}}$ to a synthetic data sample, i.e. $\bvec{\vx}_{\mathrm{g}}=G(\bvec{\vz})\in\mathcal{X}$. 

The core idea behind GAN training~\cite{goodfellow2014generative} is to set up a competing game between the discriminator and generator. The discriminator aims at respectively distinguishing $\bvec{\vx}\sim \mathbb{P}_{\mathrm{d}}$ and $\bvec{\vx}\sim \mathbb{P}_{\mathrm{g}}$ as TRUE and FAKE, i.e. performing binary classification $D:\mathcal{X}\mapsto [0,1]$. The aim of the generator, on the other hand, is to optimize $G$ such that $\mathbb{P}_{\mathrm{g}}\to \mathbb{P}_{\mathrm{d}}$, making synthetic and data samples alike to challenge the discriminator. Mathematically, the two-player game can be formulated as
\begin{align}
\min_G \max_D 
 \mathbb{E}_{\mathbb{P}_{\mathrm{d}}}\left\{\log \left[D(\bvec{\vx})\right]\right\}   + \mathbb{E}_{\mathbb{P}_{\mathrm{g}}}\left\{\log\left[1-D(\bvec{\vx})\right]\right\},\label{min-max}
\end{align}
where the inner maximum equals the JS divergence between $\mathbb{P}_{\mathrm{d}}$ and $\mathbb{P}_{\mathrm{g}}$, i.e., $D_{\mathrm{JS}}\left(\mathbb{P}_{\mathrm{d}}\Vert\mathbb{P}_{\mathrm{g}} \right)$. 



%\paragraph{Information Theory Viewpoint}\label{sec_mi}
Apart from quantifying distributions' similarity, the JS divergence has an information theory interpretation that inspires our approach presented in the next part. In accordance with the binary classification task of the discriminator, we introduce a binary random variable $s$ with a uniform distribution $\mathbb{P}_{\mathrm{s}}$. % (probability mass function). 
Associating $s=0$ and $s=1$ respectively with $\bvec{\vx}\sim \mathbb{P}_{\mathrm{d}}$ and $\bvec{\vx}\sim \mathbb{P}_{\mathrm{g}}$, we obtain a joint distribution
\begin{align}
\mathbb{P}_{\mathrm{x},\mathrm{s}}(\bvec{\vx},s) \stackrel{\Delta}{=}\left\{
\begin{array}{ll}
\mathbb{P}_{\mathrm{d}}(\bvec{\vx})\mathbb{P}_{\mathrm{s}}(s) & \text{if } s=0\\
\mathbb{P}_{\mathrm{g}}(\bvec{\vx})\mathbb{P}_{\mathrm{s}}(s) & \text{if } s=1\\
\end{array}\right..\label{def_Pxs}
\end{align}
The marginal distribution of $\mathbb{P}_{\mathrm{x},\mathrm{s}}$ with respect to $\bvec{\vx}$ (a.k.a. the mixture distribution) is equal to 
\begin{align}
\mathbb{P}_{\mathrm{m}}\stackrel{\Delta}{=}\mathbb{P}_{\mathrm{s}}(s=0)\mathbb{P}_{\mathrm{d}}+\mathbb{P}_{\mathrm{s}}(s=1)\mathbb{P}_{\mathrm{g}}= \frac{\mathbb{P}_{\mathrm{d}}+\mathbb{P}_{\mathrm{g}}}{2}.\label{Pm}
\end{align}
%$\mathbb{P}_{\mathrm{m}}$ (\ref{Pm}).
%It has the marginal with respect to $\bvec{\vx}$ equal to $\mathbb{P}_{\mathrm{m}}$ (\ref{Pm}).
Computing the mutual information of the two random variables $s$ and $\bvec{\vx}$ based on $\mathbb{P}_{\mathrm{x},\mathrm{s}}$ is identical to computing the JS divergence between $\mathbb{P}_{\mathrm{d}}$ and $\mathbb{P}_{\mathrm{g}}$, i.e.,
\begin{align} 
I(\bvec{\vx}; s)  &= \frac{E_{\mathbb{P}_{\mathrm{m}}}\left[ p_{\mathrm{d}}(\bvec{\vx})\log p_{\mathrm{d}}(\bvec{\vx})\right] + E_{\mathbb{P}_{\mathrm{m}}}\left[ p_{\mathrm{g}}(\bvec{\vx})\log p_{\mathrm{g}}(\bvec{\vx})\right]}{2}\notag\\
&=D_{\mathrm{JS}}\left(\mathbb{P}_{\mathrm{d}}\Vert\mathbb{P}_{\mathrm{g}} \right),\label{mi_js}
\end{align}

where $p_{\mathrm{d}}(\bvec{\vx})$ and $p_{\mathrm{g}}(\bvec{\vx})$ are density functions of $\mathbb{P}_{\mathrm{d}}$ and $\mathbb{P}_{\mathrm{g}}$ with respect to $\mathbb{P}_{\mathrm{m}}$.\footnote{Both $\mathbb{P}_{\mathrm{d}}$ and $\mathbb{P}_{\mathrm{g}}$ are absolutely continuous with respect to $\mathbb{P}_{\mathrm{m}}$. Therefore, their densities exist.} The minimum of the JS divergence $D_{\mathrm{JS}}\left(\mathbb{P}_{\mathrm{d}}\Vert\mathbb{P}_{\mathrm{g}} \right)$ equal to zero is attainable iff $\mathbb{P}_{\mathrm{d}}=\mathbb{P}_{\mathrm{g}}$, while zero mutual information indicates the independence between $\bvec{\vx}$ and $s$, yielding $\mathbb{P}_{\mathrm{x},\mathrm{s}}(\bvec{\vx},s)=\mathbb{P}_{\mathrm{m}}(\bvec{\vx})\mathbb{P}_{\mathrm{s}}(s)$. 


\subsection{Single-Level Augmentation} \label{subsec:1-level_aug}

Exploiting the equality presented in (\ref{mi_js}), we proceed with a systematic derivation of a progressive augmentation of GANs. %
Starting from the case of single-level augmentation with one bit $s$, we first prove the equivalence of the following two minimization problems 
\begin{align}
\min_{G} D_{\mathrm{JS}}\left(\mathbb{P}_{\mathrm{d}}\Vert\mathbb{P}_{\mathrm{g}} \right)\equiv   \min_{G} D_{\mathrm{JS}}\left(\mathbb{P}_{\mathrm{x},\mathrm{s}}\Vert \mathbb{Q}_{\mathrm{x},\mathrm{s}} \right)\label{eqv_3}
\end{align}
with $\mathbb{P}_{\mathrm{x},\mathrm{s}}$ defined in (\ref{def_Pxs}) and $\mathbb{Q}_{\mathrm{x},\mathrm{s}}$ analogously constructed as
\begin{align}
\mathbb{Q}_{\mathrm{x},\mathrm{s}}(\bvec{\vx},s) \stackrel{\Delta}{=}\left\{
\begin{array}{ll}
\mathbb{P}_{\mathrm{g}}(\bvec{\vx})\mathbb{P}_{\mathrm{s}}(s) & \text{if } s=0\\
\mathbb{P}_{\mathrm{d}}(\bvec{\vx})\mathbb{P}_{\mathrm{s}}(s) & \text{if } s=1\\
\end{array}\right..\label{def_Qxs}
\end{align}
The two joint distributions $\mathbb{P}_{\mathrm{x},\mathrm{s}}$ and $\mathbb{Q}_{\mathrm{x},\mathrm{s}}$ differ from each other by their opposite way of associating the bit $s \in \left\{0,1\right\}$ with the data and synthetic samples. %
Their marginals with respect to $\bvec{\vx}$ are identical and equal the mixture distribution $\mathbb{P}_{\mathrm{m}}$, being neither the data nor the model distribution, in contrast to the framework of \cite{ali2017}. %The equivalence proof is briefly sketched as follows:

\begin{proof}
The joint distribution $\mathbb{P}_{\mathrm{x},\mathrm{s}}$ has yielded the mutual information $\mathrm{I}(\bvec{\vx}; s)$ with the equality in (\ref{mi_js}). By analogy, we compute the mutual information $\tilde{\mathrm{I}}(\bvec{\vx}; s)$ between $\bvec{\vx}$ and $s$ which follow $\mathbb{Q}_{\mathrm{x},\mathrm{s}}$ with the equality:
\begin{align}
\tilde{\mathrm{I}}(\bvec{\vx}; s)=D_{\mathrm{JS}}\left(\mathbb{P}_{\mathrm{d}}\Vert\mathbb{P}_{\mathrm{g}} \right).\label{app:Iq}
\end{align}

The combination of (\ref{mi_js}) and (\ref{app:Iq}) leads to
\begin{align}
D_{\mathrm{JS}}\left(\mathbb{P}_{\mathrm{d}}\Vert\mathbb{P}_{\mathrm{g}} \right) = \frac{\mathrm{I}(\bvec{\vx}; s)+\tilde{\mathrm{I}}(\bvec{\vx}; s)}{2}.
\end{align}
Rewriting mutual information as KL divergence yields:
\begin{align}
D_{\mathrm{JS}}\left(\mathbb{P}_{\mathrm{d}}\Vert\mathbb{P}_{\mathrm{g}} \right) = \frac{D_{\mathrm{KL}}\left(\mathbb{P}_{\mathrm{x},\mathrm{s}}\Vert\mathbb{P}_{\mathrm{m}}\mathbb{P}_{\mathrm{s}} \right)+D_{\mathrm{KL}}\left(\mathbb{Q}_{\mathrm{x},\mathrm{s}}\Vert\mathbb{P}_{\mathrm{m}}\mathbb{P}_{\mathrm{s}}\right)}{2},\label{js_kl}
\end{align}
where $\mathbb{P}_{\mathrm{m}}$ and $\mathbb{P}_{\mathrm{s}}$ are the common marginals of $\mathbb{P}_{\mathrm{x},\mathrm{s}}$ and $\mathbb{Q}_{\mathrm{x},\mathrm{s}}$ with respect to $\bvec{\vx}$ and $s$. By further identifying
\begin{align}
\mathbb{P}_{\mathrm{m}}(\bvec{\vx}) \mathbb{P}_{\mathrm{s}}(s) = \frac{\mathbb{P}_{\mathrm{x},\mathrm{s}}(\bvec{\vx},s)+\mathbb{Q}_{\mathrm{x},\mathrm{s}}(\bvec{\vx},s)}{2}
\end{align}
and plugging it into (\ref{js_kl}), 
we finally reach to
\begin{align}
D_{\mathrm{JS}}\left(\mathbb{P}_{\mathrm{d}}\Vert\mathbb{P}_{\mathrm{g}} \right)&=D_{\mathrm{JS}}\left(\mathbb{P}_{\mathrm{x},\mathrm{s}}\Vert\mathbb{Q}_{\mathrm{x},\mathrm{s}} \right)\label{eqjoint}
\end{align}
by the definition of JS divergence. 

The above equality in (\ref{eqjoint}) implies that for any given pair $(\mathbb{P}_{\mathrm{d}},\mathbb{P}_{\mathrm{g}})$ the correspondingly constructed joint distribution pair $(\mathbb{P}_{\mathrm{x},\mathrm{s}},\mathbb{Q}_{\mathrm{x},\mathrm{s}})$ yields the same JS divergence. For this reason, we can use the two JS divergences interchangeably as the objective function while optimizing $\mathbb{P}_{\mathrm{g}}$, thereby concluding the equivalence proof for the two optimization problems in (\ref{eqv_3}). It is worth noting that the equivalence holds even if the feasible solution set of $\mathbb{P}_{\mathrm{g}}$ determined by $G$ does not include the data distribution $\mathbb{P}_{\mathrm{d}}$. This is of practical interest as it is often difficult to guarantee the fulfilment of such premise when modelling $G$. 
\end{proof}

Next, we aim to solve the equivalent problem given in (\ref{eqv_3}), following the adversary learning process behind GANs. Specifically, the objective of the discriminator $D$ converges to the estimation of the JS divergence between $\mathbb{P}_{\mathrm{x},\mathrm{s}}$ and $\mathbb{Q}_{\mathrm{x},\mathrm{s}}$
\begin{align}
\hspace{-0.2cm}\max_D \mathbb{E}_{\mathbb{P}_{\mathrm{x},\mathrm{s}}}\hspace{-0.1cm}\left\{\log \left[D(\bvec{\vx},s)\right]\right\}\hspace{-0.05cm}+\hspace{-0.05cm}\mathbb{E}_{ \mathbb{Q}_{\mathrm{x},\mathrm{s}}}\hspace{-0.1cm}\left\{\log \left[1\hspace{-0.05cm}-\hspace{-0.05cm}D(\bvec{\vx},s)\right]\right\}.\label{min-max1}
\end{align}
Comparing with the original discrimination task in GANs, i.e. (\ref{min-max}), two differences are worth noting. First, the above discriminator takes $s$ in addition to $\bvec{\vx}$. We, therefore, view $s$ as a single level of augmentation to $\bvec{\vx}$. Second, the distributions that form the TRUE/FAKE classes become $\mathbb{P}_{\mathrm{x},\mathrm{s}}$ and $\mathbb{Q}_{\mathrm{x},\mathrm{s}}$, instead of $\mathbb{P}_{\mathrm{d}}$ and $\mathbb{P}_{\mathrm{g}}$. Based on their definitions in (\ref{def_Pxs}) and (\ref{def_Qxs}), we identify $(\bvec{\vx}_{\mathrm{d}},s=0)$ and $(\bvec{\vx}_{\mathrm{g}},s=1)$ as the TRUE class, whereas $(\bvec{\vx}_{\mathrm{d}},s=1)$ and $(\bvec{\vx}_{\mathrm{g}},s=0)$ as the FAKE class. The real samples are no longer always in the TRUE class, and the synthetic samples are no longer always in the FAKE class. The correct class now depends on the combination of $\bvec{\vx}$ with the bit $s$, see Figure~\ref{fig:Data_augmentation}. %
A simple trick exists for detecting the correct class of a given pair. Namely, let the data and synthetic samples respectively convey one bit of information, with $\bvec{\vx}_{\mathrm{d}}$ encoding bit zero and $\bvec{\vx}_{\mathrm{g}}$ encoding bit one with no loss of generality. Then, the checksum of the pair $(\bvec{\vx},s)$ determines the respective class, i.e. checksum zero for TRUE and one for FAKE. \footnote{By checksum we mean the XOR operation over a bit sequence.} 


\subsection{Progressive Multi-Level Augmentation} \label{subsec:multi-level_aug}
We further extend the single-level augmentation with one bit $s$ to multi-level augmentation with an arbitrarily long random bit sequence $\bvec{\vs}$.  The two optimization problems on both sides of (\ref{eqv_3}) rely on the JS divergence to quantify the difference of two distributions. Let us replace the data and model distributions, i.e. $\mathbb{P}_{\mathrm{d}}$ and $\mathbb{P}_{\mathrm{g}}$, respectively with $\mathbb{P}_{\mathrm{x},\mathrm{s}}$ and $\mathbb{Q}_{\mathrm{x},\mathrm{s}}$. Following the same argumentation as above, we can systematically add a new bit. Repeating this procedure $L$ times will give us a bit sequence $\bvec{\vs}$ with length $L$ plus a series of equivalent problems with the same structure
\begin{align}
&\hspace{-0.25cm} \min_{G} D_{\mathrm{JS}}\left(\mathbb{P}_{\mathrm{d}}\Vert\mathbb{P}_{\mathrm{g}} \right)
\hspace{-0.05cm}\equiv  \hspace{-0.05cm} \min_{G}D_{\mathrm{JS}}\left(\mathbb{P}_{\mathrm{x},\mathbf{s}_1}\Vert \mathbb{Q}_{\mathrm{x},\mathbf{s}_1} \right)\equiv \cdots \notag\\ %\equiv  \min_{G}D_{\mathrm{JS}}\left(\mathbb{P}(\bvec{\vx},s_1,s_2)\Vert \mathbb{Q}(\bvec{\vx},s_1,s_2) \right)\notag\\
&
%\hspace{-0.25cm}  \min_{G}D_{\mathrm{JS}}\left(\mathbb{P}_{\mathrm{x},\mathbf{s}_2}\Vert \mathbb{Q}_{\mathrm{x},\mathbf{s}_2} \right)\hspace{-0.05cm} 
\cdots\hspace{-0.05cm}\equiv\hspace{-0.05cm}   \min_{G}D_{\mathrm{JS}}\left(\mathbb{P}_{\mathrm{x},\mathbf{s}_L}\Vert \mathbb{Q}_{\mathrm{x},\mathbf{s}_L} \right)
\label{eqv_4}.
\end{align}
To estimate the JS divergences in (\ref{eqv_4}), the augmented discriminator as defined in (\ref{min-max1}) now takes a bit sequence $\bvec{\vs}_l$ with $l\in\{1,\dots,L\}$ instead of the single bit $s$ (i.e., $\bvec{\vs}_{l=1}$), in addition to $\bvec{\vx}$. Following the analysis of the single bit case, it is easy to identify the remaining checksum mechanism. %
 
The consistency of the equivalences in (\ref{eqv_4}), from the zero-level (no augmentation) to single-level and then to multi-level augmentation, permits us to perform progressive augmentation, gradually increasing the augmentation level, i.e. the bit sequence length $l$. 
This is beneficial from the following aspects. 
First, the number of possible combinations of the data samples with $\bvec{\vs}_l$ grows with $l$, exponentially increasing the number of training samples and thus helping to prevent the discriminator from overfitting to the training set. 
Second, the task of the discriminator gradually becomes harder with the length $l$, as it not only needs to tell the real and synthetic samples apart but also to to understand the association rule (the checksum principle) and to learn how to separate $(\bvec{\vx},\bvec{\vs}_l)$ into $\bvec{\vx}$ and $\bvec{\vs}_l$.
Given that, progressive augmentation can be exploited during training to balance the game between the discriminator and generator whenever the former becomes too strong. 
Third, when the GAN training performance saturates at the current augmentation level, adding one random bit changes the landscape of the loss function and may boost further learning. Finally, the consistency of the checksum principle across different augmentation levels allows on-the-fly adaptation of the discriminator to the new level. We empirically illustrate the effectiveness of PA-GAN in Sec.~\ref{sec_toy_example}.

\section{PA-GAN Implementation} \label{subsec:implement}
This section addresses the integration of the progressive augmentation into the discriminator network (Sec.~\ref{subsec:network-implement}) and presents how to schedule the progression during training (Sec.~\ref{subsec:PA-schedule}). We demonstrate the benefits of the proposed augmentation in Sec.~\ref{sec_toy_example}.

\subsection{Integration into the Discriminator Network}\label{subsec:network-implement}


\begin{figure}
	%\vspace{-2em}
	\begin{center}
		\includegraphics[width=1\columnwidth]{figures/fig2_v5_3.pdf}
	\end{center}
		\vspace{-0.5em}
	\caption{\label{fig:approach} PA-GAN overview. With each level of progressive augmentation $l$ the dimensionality of $\bvec{\vs}$ is enlarged from 1 to $L$, $\bvec{\vs}=\{s_1,s_2,\dots,s_L\}$. The task difficulty of the discriminator gradually increases as the length of $\bvec{\vs}$ grows.}
		\vspace{-1em}
\end{figure}

We aim to maximally reuse existing neural network architectures tailored for GANs. 
According to the above-introduced approach and Figure~\ref{fig:approach}, the generator architecture can remain unchanged, while the discriminator network requires an alteration to incorporate the augmentation $\bvec{\vs}$.\footnote{For notation convenience, we drop the subscript of $\bvec{\vs}$ when its length is irrelevant or clear from the context.}
We apply the following changes to the discriminator network:

\paragraph{Input space augmentation}
In the proposed progressive augmentation the discrimination function $D$ takes both $\bvec{\vx}$ and $\bvec{\vs}$ as the input for checksum computation. A straightforward design is then to directly combine the sample $\bvec{\vx}$ with $\bvec{\vs}$ and feed them as input to the discriminator network. This leads to input space augmentation. 

\paragraph{Feature space augmentation}
Alternatively, we have the option to augment $\bvec{\vs}$ with the learned feature representations of $\bvec{\vx}$ attained at intermediate hidden layers. This leads to feature space augmentation.  Since only one bit information encoded by $\bvec{\vx}$ ($\bvec{\vx}_{\mathrm{d}}\leftrightarrow 1$ and $\bvec{\vx}_{\mathrm{g}}\leftrightarrow 0$) is necessary to perform the checksum computation, it is sufficient to just use high-level features of $\bvec{\vx}$ and additionally benefit from less computational effort. 

\paragraph{Augmentation mechanism}
For both cases, the way to concatenate $\bvec{\vx}$ or its feature maps with $\bvec{\vs}$ is identical. The bits $\bvec{\vs}$ are firstly assigned with the values $\{0,1\}$ before feeding them to the network. 
Then, the bit sequence $\bvec{\vs}$ is pre-processed into a form compatible with $\bvec{\vx}$.
Each of entry of $\bvec{\vs}$ creates one augmentation channel and is replicated to match the spatial dimension of $\bvec{\vx}$ or its feature maps. %
The choice of $\{0,1\}$ aims to introduce minimal changes.
When increasing the augmentation level, the new logic bit $0$ does not change the checksum. Assigning it with zero ensures no change at the layer output as well, assisting the discriminator to timely catch the change when progression takes place.  

\paragraph{Network architecture}
Depending on the augmentation space, either the input layer or the hidden layer that further processes the feature maps will additionally take care of the augmentation bits. In either case, the original layer configuration (kernel size, stride and padding type) remains except its channel size being increased by $l$. %
When a new augmentation level is reached, one extra input channel of the filter is instantiated to process the bit $l+1$. In case of passing the augmented $\bvec{\vx}$ or feature maps into a residual block, the augmentation bits are passed along with $\bvec{\vx}$ or its feature maps into the first convolutional layer in the main branch, but bypass the skip connection. All the other layers or residual blocks of the discriminator remain unchanged. 


\paragraph{Mini-batch discrimination} 
The gradients for updating $D$ are computed from the loss function given in (\ref{min-max1}), where the single bit $s$ is replaced by the bit sequence $\bvec{\vs}$. The two expectations are approximated by using mini-batches. Each mini-batch is constructed with the same number of real data samples, synthetic samples and bit sequences. %
Each bit sequence is randomly sampled and associated with one real and one synthetic sample. %
Based on the checksums of the formed pairs, we can decide their correct class and feed it into the discriminator to compute the cross-entropy loss. This way of generating $(\bvec{\vx},\bvec{\vs})$ guarantees a balanced number of TRUE/FAKE samples.


\paragraph{Non-saturating (NS) loss} 
When employing non-saturating loss for $G$ in the experiments, we follow the reformulation introduced by \cite{goodfellow2014generative}. Since the two expectation terms in (\ref{min-max1}) depend on $G$, this reformulation is applied for both of them, namely
\begin{align}
\hspace{-0.2cm}\min_G &\hspace{-0.05cm}-\hspace{-0.05cm}\mathbb{E}_{\mathbb{P}_{\mathrm{x},\mathrm{s}}}\hspace{-0.1cm}\left\{\log\hspace{-0.05cm} \left[1\hspace{-0.05cm}-\hspace{-0.05cm}D(\bvec{\vx},\bvec{\vs})\right]\right\}\hspace{-0.05cm}-\hspace{-0.05cm}\mathbb{E}_{\mathbb{Q}_{\mathrm{x},\mathrm{s}}}\hspace{-0.1cm}\left\{\log\hspace{-0.05cm} D(\bvec{\vx},\bvec{\vs})\right\}.\label{ns-loss}
\end{align}



\subsection{Progression Scheduling} \label{subsec:PA-schedule}

Bi\'nkowski et al.~\cite{Binkowski2016MMDGAN} introduced the kernel inception distance (KID) to quantify the quality of the synthetic samples on-the-fly and proposed to reduce the learning rate by tracking
the reduction of KID over iterations. %
Here we use KID to decide if the performance of $G$ at the current augmentation level saturates or even starts degrading (typically happens when $D$ starts overfitting or becomes too powerful). Specifically, after $t$ discriminator iterations, %
we compute the KID between synthetic samples and data samples drawn from the training set. %
If the current KID score is less than $5\%$ of the average of the two previous ones attained at the same augmentation level, the augmentation is leveled up, i.e. $l\rightarrow l+1$. %
To highlight the effectiveness of this scheduling mechanism we successfully exploit it for the learning rate adaptation and compare it with the proposed PA-GAN, showing the superior performance of the latter (see Sec.~\ref{subsec:ps} in the supp. material for details). 





\begin{figure}[t!]
	%\vspace{-2em}
	\begin{center}
		\includegraphics[width=0.8\columnwidth]{figures/d_g_loss_over_iterations.pdf}
	\end{center}
		\vspace{-0.5em}
	\caption{\label{fig:toy_d_g_fid_loss} Behaviour of the discriminator loss ($D$ loss) and the generator loss ($G$ loss) as well as FID changes over iterations, using SN DCGAN on CIFAR10. 
		$\mathtt{PA}$ effectively prevents the discriminator from becoming overconfident, alleviating
		the vanishing gradient issue and thus enabling continuous learning of the generator. See \ref{sec_toy_example} for details.} 	
	\vspace{-1em}
\end{figure}

\subsection{Effectiveness of Progressive Augmentation}\label{sec_toy_example}
Equipped with the implementation, we now exploit progressive augmentation with SN DCGAN~\cite{miyato2018spectral} for the image generation task on CIFAR10~\cite{Cifar10_Krizhevsky09learningmultiple} to empirically illustrate its benefits discussed in Sec.~\ref{subsec:multi-level_aug}. %
Figure~\ref{fig:toy_d_g_fid_loss} depicts the discriminator loss ($D$ loss) and the generator loss ($G$ loss) behaviour as well as changes of the FID score~\cite{FID} over iterations. It shows that the discriminator very quickly becomes over-confident, providing a non-informative backpropagation signal to train the generator and thus leading to the increase of the $G$ loss.

In order to regularize the discriminator we exploit the proposed progressive augmentation ($\mathtt{PA}$), augmenting either the input - $\mathtt{PA}\text{ }(\mathtt{input})$, or its features with spatial dimension $N/8$ - $\mathtt{PA}\text{ }(\mathtt{feat_{N/8}})$, where $N$ is the input image dimension. %
$\mathtt{PA}$ exhibits a long lasting regularization effect by means of progression and helps to maintain a healthy competition between the discriminator and the generator. 
Each rise of the $D$ loss and drop of the $G$ loss coincides with an iteration at which the augmentation level increases, and then gradually reduces after the discriminator timely adapts to the new bit.
Observing the behaviour of the $D$ and $G$ losses, we conclude that both $\mathtt{PA}\text{ }(\mathtt{input})$ and $\mathtt{PA}\text{ }(\mathtt{feat_{N/8}})$ can effectively prevent the discriminator from overfitting, alleviating
the vanishing gradient issue and thus enabling continuous learning of the generator.
At the level one augmentation, both $\mathtt{PA}\text{ }(\mathtt{feat_{N/8}})$ and $\mathtt{PA}\text{ }(\mathtt{input})$ start from the similar overfitting stage, i.e., $(a)$ and $(b)$ respectively at the iteration $60$\unit{k} and $70$\unit{k}. %
Combining the bit $s$ directly with high-level features eases the checksum computation. As a result, the $D$ loss of $\mathtt{PA}\text{ }(\mathtt{feat_{N/8}})$ reduces faster, but making its future task more difficult due to overfitting to the previous augmentation level. On the other hand,  $\mathtt{PA}\text{ }(\mathtt{input})$ let the bits pass through all layers, and thus its adaptation to augmentation progression improves over iterations. In the end, both $\mathtt{PA}\text{ }(\mathtt{feat_{N/8}})$ and $\mathtt{PA}\text{ }(\mathtt{input})$ lead to similar regularization effect and result in the improved FID scores.

For a comparison purpose, we also experiment with the $\mathtt{Dropout}$~\cite{JMLR:v15:srivastava14a} regularization applied on $\mathtt{feat_{N/4}}$ layer with the keep rate $0.7$ (the best performing rate in our experiments, see Sec.~\ref{subsec:dropout} in the supp. material for detailed comparisons). Both techniques resort to random variables for regularization. The former randomly removes features, while the latter augments them with additional random bits and adjusts accordingly the class label. %
In contrast to $\mathtt{Dropout}$, $\mathtt{PA}$ has a stronger regularization effect and leads to faster convergence (more rapid reduction of FID scores). %
In addition, we compare $\mathtt{PA}$ with the $\mathtt{Reinit.}$ baseline, where at each scheduled progression all weights are reinitialized with Xavier initialization \cite{GlorotAISTATS2010}. Compared to $\mathtt{PA}$, using $\mathtt{Reinit.}$ strategy leads to longer adaptation time (the $D$ loss decay is much slower) and oscillatory GAN behaviour, thus resulting in dramatic fluctuations of FID scores over iterations.

In addition to Figure~\ref{fig:toy_d_g_fid_loss}, we have also designed a toy example for an empirical investigation on the effectiveness of progressive augmentation, see Sec.~\ref{sup_sec_toy_example} in the supp. material. The attained observation is in line with that of Figure~\ref{fig:toy_d_g_fid_loss}.

